RoPE Attention Can Be Trained in Almost Linear Time

The Rotary Position Embedding (RoPE) mechanism has become a powerful enhancement to the Transformer architecture, which enables models to capture token relationships when encoding positional information. However, the RoPE mechanisms make the computations of attention mechanisms more complicated, which makes efficient algorithms challenging. Earlier research introduced almost linear time algorithms for the forward computation under specific parameter settings of bounded entries (i.e., in time $n^{1+o(1)}$ where $n$ is the number of input tokens), but has not addressed backward computation. In this work, we develop the first almost linear time algorithm for backward computations in the RoPE-based attention under bounded entries. Our approach builds on recent advancements in fast RoPE attention computations, utilizing a novel combination of the polynomial method and the Fast Fourier Transform. Furthermore, we show that with lower bounds derived from the Strong Exponential Time Hypothesis (SETH), the bounded entry condition is necessary for subquadratic performance.

==> 61_impact.tex <==
\section{Impact Statement} \label{sec:impact}

We introduce the first almost linear time algorithm for backward gradient computation in RoPE attention, advancing both theoretical understanding and computational efficiency for large-scale transformers. As this is a theoretical contribution, we do not foresee any potential negative societal impacts.
